Affine Monads and Lazy Structures for Bayesian Programming

We show that streams and lazy data structures are a natural idiom for programming with infinite-dimensional Bayesian methods such as Poisson processes, Gaussian processes, jump processes, Dirichlet processes, and Beta processes. The crucial semantic idea, inspired by developments in synthetic probability theory, is to work with two separate monads: an affine monad of probability, which supports laziness, and a commutative, non-affine monad of measures, which does not. (Affine means that $T(1)\cong 1$.) We show that the separation is important from a decidability perspective, and that the recent model of quasi-Borel spaces supports these two monads. To perform Bayesian inference with these examples, we introduce new inference methods that are specially adapted to laziness; they are proven correct by reference to the Metropolis-Hastings-Green method. Our theoretical development is implemented as a Haskell library, LazyPPL.

==> gps.tex <==

\label{sec:hardexamples}

We demonstrate the power of laziness for constructing models, illustrating more examples from the theory of Bayesian non-parametrics and practical probabilistic programming.

\subsection{Laziness, control flow and addressing}
\label{sec:hardexamples:addressing}
 We consider a very simple model, to illustrate the kind of reorganization that laziness allows.
Suppose that we toss a fair coin, and then, depending on the outcome, we toss one of two biased coins. We then notice that we got the same result both times.
What was the result? 
\begin{lstlisting}
 model :: Prob (Bool, Bool)
 model = do x <- bernoulli 0.5
            y <- if x then bernoulli 0.4 else bernoulli 0.7
            return (x,y)
 test = do {(x,y) <- sample model; score (if x==y then 1 else 0); return x}
\end{lstlisting}
The result is \lstinline|True| with probability $\frac{0.5\times 0.4}{0.5 \times 0.7}\approx 0.57$.
   Because the probability monad is affine, the model is equivalent to the situation where we actually tossed all three coins: by laziness, only two coins will only ever actually be looked at on any run. 
\begin{lstlisting}
 model2 = do x <- bernoulli 0.5
             ytrue <- bernoulli 0.4
             yfalse <- bernoulli 0.7
             return (if x then (x, ytrue) else (x, yfalse)) 
\end{lstlisting}
Although the second formulation might look more costly, in fact the run time cost is roughly the same, because of laziness, and moreover, it results in fewer rejections with our new Metropolis-Hastings kernel 
(\S\ref{sec:msmh:rose}).
This is because in the second formulation, all three bernoulli statements are allocated different nodes in the rose tree, and so 
the proposal will often be accepted even if just \lstinline|x| changes. 
In the first formulation, however, the proposal will be rejected unless both \lstinline|x| and \lstinline|y| are changed simultaneously. 
These kinds of `addressing' issues have been noted by other authors (e.g~\cite{kiselyov-problems}), and we note that laziness provides a clear way to deal with them. 

\subsection{Regression with a prior over program expressions}
\label{sec:hardexamples:progind}

We revisit the regression scenario from Section~\ref{sec:easyexamples:reg}. We can phrase program induction as a regression problem.
This is done in e.g.~\cite{meent-book}, but we discuss it here because the typed setting is clarifying, and it illustrates some further aspects of laziness. 
We consider a prior over program expressions, \lstinline|randExpr :: Prob Expr|, an evaluation function \lstinline|Expr -> RealNum -> RealNum|,
and then calling
\begin{lstlisting}
  regress sigma dataset (do { e <- randExpr ; return (eval e) })
\end{lstlisting}
We used this method to infer the expressions shown in Figure~\ref{fig:regression}.
In more detail, but keeping things fairly simple, we consider a datatype
\begin{lstlisting}
  data Expr = Var | Constt RealNum | Add Expr Expr | Mult Expr Expr
            | IfLess RealNum Expr Expr
\end{lstlisting}
for expressions with a single variable, and consider an evaluation function \lstinline|Expr -> RealNum -> RealNum|
defined by induction over expressions.
It remains for us to discuss our prior, which is a random expression built by recursively making choices about what its subexpressions will be. 
%A first attempt at a random expression is by building an expression, making random choices about what its subexpressions will be. 
%\begin{lstlisting}
%randExpr':: Prob Expr
%randExpr' = do
%  -- choose what kind of expression we'll have (variable, constant, addition)
%  i <- categorical [0.3,0.3,0.18,0.18,0.04]
%  -- choose any parameters it needs, and generate subexpressions
%  e <- [return Var ,
%        do { n <- normal 0 5 ; return $ Constt n },
%        do { e1 <- randExpr' ; e2 <- randExpr' ; return $ Add e1 e2},
%        do { e1 <- randExpr' ; e2 <- randExpr' ; return $ Mult e1 e2},
%        do { r <- normal 0 5 ; e1 <- randExpr' ; e2 <- randExpr' ; return $ IfLess r e1 e2}]
%       !! i        
%  return e
%\end{lstlisting}
Here we use the method of Section~\ref{sec:hardexamples:addressing}, exploiting laziness to simultaneously consider all the possible expression choices, which are now infinite. 
\begin{lstlisting}
 randExpr :: Prob Expr
 randExpr = do
   i <- categorical [0.3,0.3,0.18,0.18,0.04]
   es <- sequence
      [return Var ,
      do { n <- normal 0 5 ; return $ Constt n },
      do { e(*@$_1$@*) <- randExpr ; e(*@$_2$@*) <- randExpr ; return $ Add e(*@$_1$@*) e(*@$_2$@*)},
      do { e(*@$_1$@*) <- randExpr ; e(*@$_2$@*) <- randExpr ; return $ Mult e(*@$_1$@*) e(*@$_2$@*)},
      do { r <- normal 0 5 ; e(*@$_1$@*) <- randExpr ; e(*@$_2$@*) <- randExpr ;
           return $ IfLess r e(*@$_1$@*) e(*@$_2$@*)}]
   return $ es !! i
\end{lstlisting}
When we run inference, each expression template (roughly a `sketch',~\cite{sketching})  is allocated a different path through the rose tree. Some likely results are shown in Fig.~\ref{fig:dp}(b).

\subsection{General stochastic memoization}
\label{sec:hardexamples:stochmem}
%\todo{Could drop if insufficient space}
In Section~\ref{sec:easyexamples:stochmem} we discussed stochastic memoization, a second-order function 
\lstinline|memoize|,
which is a crucial primitive in Church~\cite{goodman:church}. 
Memoization is a form of laziness, and conversely, as we discussed, it can be defined in using pure laziness for many specific types. An alternative approach is to actually use a memo table, and then we can define 
\lstinline|memoize| whenever its argument supports equality testing. We define 
\begin{lstlisting}
generalMemoize :: Eq a => (a -> Prob b) -> Prob (a -> b)
\end{lstlisting}
Our implementation ensures that a sample from \lstinline|generalMemoize f| returns a function that has a fresh hidden memo table of pairs \lstinline|(x,y)| of argument/result pairs, initialized empty. When
the function is subsequently called with argument \lstinline|x|:
\begin{itemize}
\item If a value at \lstinline|x| is already stored in the memo table, return that value.
\item If not, \lstinline|x| sample 
 \lstinline|y <- f x|, store \lstinline|(x,y)| in the memo table, and return
  \lstinline|y|.
\end{itemize}
To work with this memo table, we need to use state. (We do this via \lstinline|unsafePerformIO|.) Our implementation is safe in the following sense:
\begin{itemize}
\item the sampled function appears deterministic to the user: function calls can be reordered, discarded, and copied~\cite{Fuhrmann}; and
\item the resulting distribution (\lstinline|generalMemoize f|) in \lstinline|(Prob (a -> b))| satisfies the commutativity and affine laws (\ref{eqn:comm}, \ref{eqn:affine}).
\end{itemize}
As a simple example, we can define white noise via 
\begin{lstlisting}
 generalMemoize (\x -> uniform) :: Prob (RealNum -> RealNum)
\end{lstlisting}
White noise is difficult to analyze in measure-theoretic terms, and it is curious that this coincides with the limitations of pure laziness in functional programming. 
\subsection{Regression with a Gaussian process}
\label{sec:hardexamples:gp}

Gaussian processes (GPs) are examples of random real-valued functions, so their type in LazyPPL is \lstinline|Prob (a -> RealNum)|.  To illustrate the key points, we have focused on a very simple Gaussian process, the one-dimensional Wiener process, also known as Brownian motion. This has type \lstinline|Prob (RealNum -> RealNum)|.

%\todo[inline]{Not sure if the following paragraph is needed.}Gaussian processes are often described as random functions.
%If $\Omega$ is the basic probability space, then a random function $T\to \RR$ is a function $X : \Omega \times T \to \RR$;
%a GP is one such that the random variable for any $(t_1, \dots, t_n) \in T^n$ the joint random variable  $(X(t_1), \dots, X(t_n))$ is distributed as a multivariate normal on $\RR^n$. (In particular each $X(t)$ is normally distributed.)
%In our formalism, random functions are just functions \lstinline|Prob (T -> RealNum)|, and so a Gaussian process can be described as
%a random function \lstinline|gp :: Prob (T -> RealNum)| such that
%\begin{lstlisting}
%do { f <- gp ; return (f t1,...,f tn) } :: (RealNum,...RealNum)}
% \end{lstlisting}
%is a multivariate normal. 

A draw from the Wiener process is a function that is almost surely continuous everywhere but differentiable nowhere. Informally, the Wiener process is the continuous-time version of a symmetric random walk on $\RR$, starting at 0. We have used this as a prior for a regression model, using the \lstinline|regress| function and the dataset from Section~\ref{sec:easyexamples:reg}. See Figure~\ref{fig:regression} (right) for some draws from the posterior. 

Although the Wiener process formally involves an uncountable number of random choices, in practice for Wiener process regression we only need to know its value at the points where it is evaluated. These depend on the observation points, the resolution of the plot, and the viewport. Thus although we use the Wiener process as a random function, it makes practical sense because it can be evaluated lazily. 

The Wiener process challenges our primitives for laziness. Before turning to our implementation of the Wiener process, we first discuss a simpler discrete Gaussian random walk, \lstinline|Prob (Int -> RealNum)|. At each step, this moves according to a normal distribution. This might be defined as
\begin{lstlisting}
rw :: Prob (Int -> RealNum)
rw = do { ys <- iterateM (\y -> normal y 1) 0 ; return (\x -> ys !! x) }
\end{lstlisting}
Suppose we subsequently evaluate the position at $1$ then $5$ and then $3$:
\begin{lstlisting}
do {f <- rw ; (f 1 , f 5, f 3)}
\end{lstlisting}
This implementation is lazy -- it will never actually make the random choices needed to determined
the position at time $6$. But it will need to calculate the position at times $2$ and $4$. 
In fact, it is possible to avoid these by following the \emph{Brownian bridge} method (e.g.~\cite[\S3.1.1, Fig.~ 3.1]{brownian-bridge}):
\begin{lstlisting}
do f(*@$_1$@*) <- normal 0 1
   f(*@$_5$@*) <- normal 0 (sqrt 2)
   f(*@$_3$@*) <- normal (f(*@$_1$@*) + 0.5*(f(*@$_5$@*)-f(*@$_1$@*))) 1
   return (f(*@$_1$@*) , f(*@$_5$@*), f(*@$_3$@*))
\end{lstlisting}
We can also implement the Brownian bridge method without knowing in advance which arguments a function will be called with. Somewhat similarly to \S\ref{sec:hardexamples:stochmem}, our implementation is to return a function that has a hidden memo table of pairs \lstinline|(x,y)| of argument/result pairs, initialized with one entry \lstinline|(0,0)|. When
the function is subsequently called with argument \lstinline|x|:
\begin{itemize}
\item If a value at \lstinline|x| is already stored in the memo table, return that value.
\item If not, and if \lstinline|x| is lower than the lowest entry \lstinline[mathescape]|(x$_0$, y$_0$)|, or higher than the highest entry \lstinline[mathescape]|(x$_0$, y$_0$)|, sample 
 \lstinline[mathescape]+y <- normal y$_0$ (sqrt |x$_0$ - x|)+, store \lstinline|(x, y)| in the memo table, and return
  \lstinline|y|.
\item Otherwise, if \lstinline[mathescape]|(x$_0$, y$_0$)| and \lstinline[mathescape]|(x$_1$, y$_1$)| are the nearest points in the memo table ($\mlstinline{x$_0$}\leq \mlstinline{x}\leq \mlstinline{x$_1$}$), then
  sample 
  \lstinline[mathescape]|y <- normal (y$_0$ + r*(y$_1$ - y$_0$)) (sqrt (r * (x$_1$ - x)))|, and store \lstinline|(x, y)| in the memo table, and return \lstinline|y|.
  Here \lstinline[mathescape]|r = (x - x$_0$)/(x$_1$ - x$_0$)|.
\end{itemize}
%\todo[inline]{A cartoon of this might be nice, if there is time/space.}
To store the memo table, we need to use state (via \lstinline|unsafePerformIO|). Our implementation is safe in the same sense as the stateful stochastic memoization (\S\ref{sec:hardexamples:stochmem}): the sampled function appears deterministic to the user, and the resulting distribution \lstinline|Prob (Int -> RealNum)| satisfies the commutativity and discardability laws.

This exact same pseudocode works for the Wiener process, and this is how we implement
\lstinline|wiener :: Prob (RealNum -> RealNum)|.
In the case of functions from the integers, this Brownian bridge implementation is more efficient than the list based implementation \lstinline|rw|. But in the Wiener process,
which takes real valued arguments, there appears to be no other way to implement this random function.
Thus `continuous' stochastic processes, which push against the measure-theoretic foundations of probability,
also push against the traditional lazy foundations of functional programming. 




\subsection{Feature extraction and the Indian Buffet Process}
\label{sec:hardexamples:ibp}

A \emph{feature assignment} for a data set is a finite set of features, together with a subset of these features for each data point. For example we can have a set of movies, and a feature assignment could be a set of genres for each movie. We can represent a feature assignment as a boolean-valued matrix, where the columns are features and the rows are data points.  

We consider the problem of feature extraction, where we have a data set but the features are unknown. We can view this as a generalized version of the clustering problem where clusters are allowed to overlap, so a data point could belong to many clusters. 

The Indian Buffet Process (IBP) is a Bayesian model for feature extraction \cite{ibp}. It provides a distribution on boolean-valued matrices, described by a process for sampling rows one by one. As with the CRP, we think of data points as customers walking into a restaurant, but here each customer selects a number of dishes (features) from a buffet. The dishes are selected based on their popularity with previous customers. To implement the IBP we use some abstract types:
\begin{lstlisting}
newtype Restaurant = R ([[Bool]], Counter)  
newtype Dish       = D Int  deriving (Eq, MonadMemo Prob)
newRestaurant :: RealNum -> Prob Restaurant 
newCustomer   :: Restaurant -> Prob [Dish]       
\end{lstlisting}
The idea is that a restaurant is initialized with an infinite matrix describing an  infinite (but lazy) simulation of the process. The counter keeps track of how many rows have already been consumed by customers coming in. A call to (\lstinline|newCustomer r|) will simply look up the next row in the matrix, return the column indices containing 1's, and increment the counter in \lstinline|r|. 

\paragraph*{A probabilistic counter.} The \lstinline|Counter| type is introduced to encapsulate an integer reference:
\begin{lstlisting} 
data Counter = C (IORef Int)
\end{lstlisting}
The main reason for this encapsulation is to hide and restrict any stateful operations in the modelling interface. Although our use of state is safe in practice, the counter will affect the distributions, so all operations are probabilistic:
\begin{lstlisting}
newCounter       :: Prob Counter
readAndIncrement :: Counter -> Prob Int 
\end{lstlisting}
 \begin{wrapfigure}[16]{r}{4.3cm}\vspace{-3.2em}
\includegraphics[scale=0.2]{IBPpicture.pdf}
\vspace{-3.2em}
\caption{\label{fig:ibp}Feature extraction for a psychological experiment. The columns correspond to features and assignments are automatically inferred using an IBP model.}
\end{wrapfigure}
It is notable that the IBP seems to necessitate some deviation from pure laziness in its implementation, which appears to coincide with continuity issues in the analysis of the IBP (e.g.~\cite[Sl.~6]{roy-ibp}, also~\cite{Roy-ChurchNP,roy2014continuum,aafrr-comput-cond-ind}).
(We note that a counter can be useful for other models, beyond the IBP, to keep track of the process history. One example is an alternative representation of the Chinese Restaurant Process in which a new customer is assigned a table based on the locations of previous customers.) 
% (In Section~\ref{} we used stick-breaking instead, avoiding the need for state.) 

\paragraph*{A feature extraction example.} We turn to an application of the IBP. We have used LazyPPL to solve a basic problem from applied psychology \cite{navarroNonparametricBayesianMethod2006}. The problem is as follows. We have a set of 16 countries together with a similarity coefficient for each pair of distinct countries, calculated based on answers from participants in a study.  
The goal is to infer a set of underlying features which characterize the countries in the participants' minds, and influence their judgement. In the Bayesian model we consider, the similarity coefficients are calculated from the subset of features that two countries share. We use an IBP prior on feature assignments for the set of countries, and incorporate the experimental data to infer a distribution on probable feature assignments. 


Our results are similar to those in \cite{navarroNonparametricBayesianMethod2006}, surprisingly so since we just used the plain inference of Section~\ref{sec:msmh}. The features are inferred and abstract, but they are interpretable. For example, in Fig.~\ref{fig:ibp}, columns 1 and 5 could correspond to Asia and Caribbean respectively; column~7 could indicate conflicts.  


\subsection{Relational modelling and Mondrian process}
\label{sec:hardexamples:mondrian}

As a final example, we consider the Mondrian process~\cite{royMondrianProcess2009}, a model often used to generate random relations between sets.
Formally, a draw from a Mondrian process is a block partition of a $k$-dimensional hypercube of the form $\Theta_1 \times \dots \times \Theta_k$, where each $\Theta_d$ is a closed interval $[a_d, b_d]$. 
% We will use it to model $k$-dimensional relations $\Theta_1 \times \dots \times \Theta_k \to \{\texttt{true}, \texttt{false}\}$.
% The Mondrian process can be seen as a $k$-dimensional generalization of the Poisson process.
% Due to its convenient self-consistency property,
(see also~\cite{bentleyMultidimensionalBinarySearch1975}). These are easy to manipulate with Haskell data types: 
\begin{lstlisting}[escapechar=@]
data Mondrian a = Block a [(RealNum, RealNum)]
    | Partition Int RealNum [(RealNum, RealNum)] (Mondrian a) (Mondrian a)
\end{lstlisting}
Our implementation of the Mondrian process provides a parameterized sampler:
\begin{lstlisting}[escapechar=@]
newMondrian :: (Prob a) -> RealNum 
                            -> [(RealNum, RealNum)] -> Prob (Mondrian a)
\end{lstlisting}
A call to (\lstinline|newMondrian| $\mu\ \lambda\ \Theta$) follows a recursive process, %very amenable to a functional implementation,
which we summarize now. 

The intuitive idea is that we make one cut through the hypercube $\Theta$, and then recursively call the Mondrian process on each separate part.  The parameter $\lambda \in \RR$ is a fixed budget, which determines how deep the recursion will go. Every cut takes away some amount from the budget, sampled from an exponential distribution, and we stop when the budget has run out. The direction of the cut is orthogonal to one of the axes, chosen  at random with probability proportional to the length of the corresponding interval $[a_d, b_d]$. Then, we draw a point uniformly in $[a_d, b_d]$ to determine the cut position. This yields a $k$-d tree, whose leaves are $k$-dimensional blocks partitioning the initial domain $\Theta$ (the root of the tree) and whose internal nodes are given by a cut point $x_d \in \RR$ splitting a subdomain $\Theta' \subseteq \Theta$ across a given axis $d \in \NN$ (\emph{cf.} the \lstinline|Mondrian| data type). Interestingly, in dimension $k = 1$ the positions of the cuts form a Poisson point process (\S\ref{sec:intro:poisson}).

% Such a generative process $M(\lambda, \Theta_1, \dots, \Theta_k)$ partitions the $k$-dimensional hypercube as follows. At each recursive step, we sample the next residual time $t$ at which a cut $x_d$ -- orthogonal to one of the axes in a dimension $d \in \{1, \dots, k\}$ to be determined -- will occur. Each axis $\Theta_d = [a_d, b_d]$ is then thought of as an independent clock whose residual time until ringing is exponentially distributed with rate its length $b_d - a_d$. In this competing exponential clock setting, the residual time $t$ until one of the clocks rings is exponentially distributed with rate the sum of the lengths $\sum_{d=1}^k b_d - a_d$, and the probability that the $d$-th clock $\Theta_d$ be the first one to do so is proportional to $b_d - a_d$. If $t$ exceeds the budget $\lambda$, we stop there and return the block $\Theta_1 \times \dots \times \Theta_k$. Otherwise, we cut the domain orthogonally to the $d$-th axis at $x_d$, and recurse with remaining budget $\lambda - t$ on a left (resp. right) subdomain where $\Theta_d$ has been restricted to $[a_d, x_d]$ (resp. $[x_d, b_d]$) and the other dimensions are left unchanged.

After generating the partition, we annotate each block with a sample $p$ from the parameter distribution $\mu$. Typically, $\mu$ is a distribution on $[0, 1]$ so that $p$ represents the probability that points associated with this block should be related. (In two dimensions and for $\Theta = [0, 1]^2$, we have a particular kind of \emph{graphon}, see e.g.~\cite{orbanz-roy}.)

\paragraph*{Experiments with a generative model for relational data.}
Following \cite{royMondrianProcess2009}, we have experimented with Mondrian process inference using a synthetic data set, consisting of relational data generated from an actual 1921 painting by Piet Mondrian (Figure~\ref{fig:mondrian} (a,b)). This is intended as a simple proof of concept. The implementation relies on a function for generating relations lazily:
 \begin{lstlisting}
sampleRelationFromMondrian2D :: Mondrian RealNum -> Prob Relation
\end{lstlisting}
\lstinline|Relation| is a type of lazy infinite binary relations, or matrices. We define  abstract types \lstinline|Row| and \lstinline|Col| and obtain an interface for modelling with exchangeable arrays:
\begin{lstlisting}
data Relation = Relation Counter Counter [[Bool]]
newRow :: Relation -> Prob Row
newCol :: Relation -> Prob Col
lookup :: Relation -> Row -> Col -> Bool
\end{lstlisting}
An example posterior sample is displayed in Figure~\ref{fig:mondrian} (c). We can experiment with variants of this model. For instance, if we record the plane coordinates when creating our synthetic data points, our inference algorithm recovers block partitions analogous to the initial painting (Figure~\ref{fig:mondrian} (d)).

\subsection{Summary}
Probabilistic programming makes it easy to construct hierarchies or combinations of models. This is especially true in LazyPPL where the types and lazy data structures make the modularity clear. 

We emphasize that laziness can be exploited at every level: for instance it is easy to generate a Mondrian relation over the tables of a Chinese Restaurant for a dataset, even without knowing in advance how many tables there are. There are many practical examples of this kind of construction:  Mondrian Forests \cite{lakshminarayananMondrianForestsLargeScale2016}, Chinese Restaurant Franchises \cite{blei2010nested}, hierarchical Generalized IBPs \cite{roy2014continuum}, and others. 
For these complex models it is harder to reason about symmetries and exchangeability, so abstract types for encapsulating internal details are another benefit of LazyPPL.


% \todo[inline]{working on punchy summary below. mention Mondrian forest and IRM etc.}


% This is especially true in LazyPPL

% LazyPPL makes it easy to experiment and prototype variants  


% Other examples our interface will support in future versions will be inference (with visualization) of 3D relations, the Mondrian forest algorithm~\cite{lakshminarayananMondrianForestsEfficient2015,lakshminarayananMondrianForestsLargeScale2016} for regression and classification, and making use of lazy Mondrians in the Infinite Relational Model~\cite{kempLearningSystemsConcepts2006}.





% , which will be the hyperparameter of a distribution $\nu$ from which we will sample the truth value of the relation we model at this given block. 




% This results in the following abstract type and generative process in \lstinline|Mondrian.hs|.:

% \begin{lstlisting}[escapechar=@]
% newMondrian (@$\mu$@:: Prob a) (@$\lambda$@:: RealNum) (@$\Theta$@:: [(RealNum, RealNum)]) 
%   :: Prob (Mondrian a)
% \end{lstlisting}

% The sampling distribution $\nu$ will typically be \lstinline|bernoulli| for example: each block is then equipped with a bias $p$ and $k$ elements (a point in the block) will be related with probability $p$. This leads to the following implementation when $k = 2$ (taking advantage of laziness, the $y$-axis (resp. $x$-axis) of a 2D block is thought of as the row (resp. column) of a (potentially infinite) matrix.

% \begin{lstlisting}[escapechar=@]
% sampleRelationFromMondrian2D :: Mondrian RealNum -> Prob Matrix
% sampleFiniteRelationFromMondrian2D :: Mondrian RealNum -> Int 
%   -> Prob (Map (RealNum, RealNum) Bool)
% % \end{lstlisting}

% As an example, inspired from \cite{royMondrianProcess2009}, we try to infer a relation stemming from an actual 1921 painting of Piet Mondrian, by observing finite binary relations randomly generated from it~(\ref{fig:regression}). 

\begin{figure}
  \raisebox{1em}{\includegraphics[scale=0.07]{mondrian1921.png}}\quad 
  \includegraphics[scale=0.2]{pietMondrian-plus-relation.pdf}\quad 
    \includegraphics[scale=0.2]{mondrian-relation-matrix.pdf}\quad
  % \includegraphics[scale=0.2]{mondrian-relation_0.pdf}\quad 
   \includegraphics[scale=0.2]{mondrian-relation_2.pdf}
  \caption{\label{fig:mondrian}Left to right: (a)~``\emph{Composition with Large Blue Plane, Red, Black, Yellow, and Gray}'' by Mondrian (1921), (b)~ our representation of (a), and a random synthetic relation (red = \texttt{false} for a pair of points, green = \texttt{true}), (c) a posterior sample, 
  and (d)~ a variant of the experiment recording the plane coordinates.}
\end{figure}






% it has been successfully used in machine learning as a form of decision tree to define a new class of random forests (called \emph{Mondrian forests}), achieving competitive performance in online non-parametric classification~\cite{lakshminarayananMondrianForestsEfficient2015} and large-scale regression~\cite{lakshminarayananMondrianForestsLargeScale2016,balogMondrianProcessMachine2015}. The Mondrian process has also been used as an applied modeling tool -- e.g. in computational biology, in conjunction with a Bayesian hierarchical regression model, to recover species interactions from the ecological system they live in~\cite{aderholdReconstructingEcologicalNetworks}. 













%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> typed-examples.tex <==
\todo[inline]{Rewrite more in the style of a specification e.g. \eqref{eqn:gp}?}

\subsection{Chinese restaurant process and abstract data types}
\label{sec:easyexamples:crp}
The random partition of the data set arising from the stick-breaking construction above is called a \emph{Chinese restaurant process} (CRP) (e.g.~\cite{gv-bnp}). The idea is to think of data points as customers arriving into a restaurant. Each customer is assigned a table, and so tables correspond to clusters. 

The stick-breaking construction is only one possible implementation of the CRP.
% another typical one assigns a table to a new customer with probability proportional to the current number of customers at that table.
There is also no requirement that tables should be represented as integers. We find it useful to encapsulate our representations using abstract data types: 
\begin{lstlisting}
 newtype Restaurant = R [RealNum]
 newtype Table      = T Int deriving (Eq,MonadMemo Prob)
\end{lstlisting}
These come with constructors: 
\begin{lstlisting}
 newRestaurant :: RealNum -> Prob Restaurant   
 newCustomer   :: Restaurant -> Prob Table 
\end{lstlisting}
For our specific implementation, \lstinline|(newRestaurant| $\alpha$\lstinline|)| just performs the stick-breaking, and \lstinline|(newCustomer r)| draws a random stick  with probability equal to its length. 

This abstract interface prevents the programmer from accessing the underlying representation. This is important, because we want to remove the artificial ordering on clusters to preserve \emph{statistical exchangeability}: the idea that data points can be considered in any order and the distribution of the partition does not change (e.g.~\cite{xrp-data,staton:betabernoulli}). Although the implementation of \lstinline|Table| is hidden, notice that we retain the fact that it supports memoization.

With this interface, the cluster assignment function has a clear implementation:
\begin{lstlisting}
 assignClusters :: RealNum -> [a] -> Prob [(a, Table)]  
 assignClusters (*@$\cb\alpha$@*) dataset = do
    r <- newRestaurant (*@$\cb\alpha$@*) 
    mapM (\x -> (x, newCustomer r)) dataset
\end{lstlisting}

Regression and clustering are widely studied problems, but we already see the power of laziness and types at this level. In LazyPPL we can seamlessly manipulate complex or infinite-dimensional distributions. We will explore this with more advanced examples in Section~\ref{sec:hardexamples}.

%can first use \lstinline|dp| to assign a fresh name (guid) to each cluster, and then assign various facets to each named cluster. 


%The Dirichlet process is a basic non-parametric model, but it is easy to compose the code here to explore hierarchical Dirichlet processes and so on.

% \paragraph{Technical point.} Memoization is not fully natively supported in Haskell at present (although see~\cite{Hinze00memofunctions}), and so we implemented \lstinline|memoize| by building a private cache. This is a few lines of `unsafe IO' code, whereas everything else is purely functional, but this is entirely encapsulated within the definition of \lstinline|memoize|. 

% \emph{Feature extraction} is a generalization of clustering, where each point can belong to more than one feature. For example, a movie belongs to multiple genres. We have used laziness in LazyPPL to implement the Indian Buffet Process~\cite{ibp}, which supports an unbounded number of features.  

\subsection{Feature extraction and the Indian Buffet Process}
\label{sec:hardexamples:ibp}


% The model is based on the Indian Buffet process, which can also be explained in terms of the Beta process and the Bernoulli process. 
% The statistical model~\cite{} is given by 
% \[
%   P \sim \mathcal{B}\mathit{eta}\mathcal{P}\mathit{rocess}
% \qquad
% F_i\sim \mathcal{B}\mathit{ernoulli}\mathcal{P}\mathit{rocess}(P)
% \]
% Here $P$ is a latent variable describing the underlying features and their connections, and $F_i$ is a random variable for each data point, itself a finite set of features. 



\iffalse


A \emph{feature assignment} for a data set is a finite set of features, together with a subset of these features for each data point. For example we can have a set of movies, and a feature assignment could be a set of genres for each movie. We can represent a feature assignment as a boolean-valued matrix, where the columns are features and the rows are data points.  

We consider the problem of feature extraction, where we have a data set but the features are unknown. We can view this as a generalized version of the clustering problem where clusters are allowed to overlap, so a data point could belong to many clusters. 

The Indian Buffet Process (IBP) is a Bayesian model for feature extraction \cite{ibp}. It provides a distribution on boolean-valued matrices, described by a process for sampling rows one by one. As with the CRP, we think of data points as customers walking into a restaurant, but here each customer selects a number of dishes (features) from a buffet. The dishes are selected based on their popularity with previous customers. To implement the IBP we use some abstract types:
\begin{lstlisting}
newtype Restaurant = R ([[Bool]], Counter)  
newtype Dish       = D Int  deriving (Eq, MonadMemo Prob)
newRestaurant :: RealNum -> Prob Restaurant 
newCustomer   :: Restaurant -> Prob [Dish]       
\end{lstlisting}
The idea is that a restaurant is initialized with an infinite matrix describing an  infinite (but lazy) simulation of the process. The counter keeps track of how many rows have already been consumed by customers coming in. A call to (\lstinline|newCustomer r|) will simply look up the next row in the matrix, return the column indices containing 1's, and increment the counter in \lstinline|r|. 

\paragraph*{A probabilistic counter.} The \lstinline|Counter| type is introduced to encapsulate an integer reference:
\begin{lstlisting} 
data Counter = C (IORef Int)
\end{lstlisting}
The main reason for this encapsulation is to hide and restrict any stateful operations in the modelling interface. Although our use of state is safe in practice, the counter will affect the distributions, so all operations are probabilistic:
\begin{lstlisting}
newCounter       :: Prob Counter
readAndIncrement :: Counter -> Prob Int 
\end{lstlisting}
 \begin{wrapfigure}[16]{r}{4.3cm}\vspace{-3.2em}
\includegraphics[scale=0.2]{IBPpicture.pdf}
\vspace{-3.2em}
\caption{\label{fig:ibp}Feature extraction for a psychological experiment. The columns correspond to features and assignments are automatically inferred using an IBP model.}
\end{wrapfigure}
It is notable that the IBP seems to necessitate some deviation from pure laziness in its implementation, which appears to coincide with continuity issues in the analysis of the IBP (e.g.~\cite[Sl.~6]{roy-ibp}, also~\cite{Roy-ChurchNP,roy2014continuum,aafrr-comput-cond-ind}).
(We note that a counter can be useful for other models, beyond the IBP, to keep track of the process history. One example is an alternative representation of the Chinese Restaurant Process in which a new customer is assigned a table based on the locations of previous customers.) 
% (In Section~\ref{} we used stick-breaking instead, avoiding the need for state.) 

\paragraph*{A feature extraction example.} We turn to an application of the IBP. We have used LazyPPL to solve a basic problem from applied psychology \cite{navarroNonparametricBayesianMethod2006}. The problem is as follows. We have a set of 16 countries together with a similarity coefficient for each pair of distinct countries, calculated based on answers from participants in a study.  
The goal is to infer a set of underlying features which characterize the countries in the participants' minds, and influence their judgement. In the Bayesian model we consider, the similarity coefficients are calculated from the subset of features that two countries share. We use an IBP prior on feature assignments for the set of countries, and incorporate the experimental data to infer a distribution on probable feature assignments. 


Our results are similar to those in \cite{navarroNonparametricBayesianMethod2006}, surprisingly so since we just used the plain inference of Section~\ref{sec:msmh}. The features are inferred and abstract, but they are interpretable. For example, in Fig.~\ref{fig:ibp}, columns 1 and 5 could correspond to Asia and Caribbean respectively; column~7 could indicate conflicts.  
\fi 

%%% Local Variables: 
%%% TeX-master: "paper"
%%% End:
%%% reftex-default-bibliography: ("refs.bib")

